Investigating model influence on the analytical resolution of neutron reflectometry

Neutron reflectometry is a critical tool for investigating the structure of thin films and interfaces. However, the misapplication of the Born approximation to reflection geometry leads some to assume that the minimum thickness that may be probed by neutron reflectometry is limited by the Q-range of the measurement. In this study, we use model-dependent analysis, multiple isotopic contrasts, and magnetic spin states, to show that it is possible to resolve structures significantly smaller than this perceived limit. To quantify this "analytical resolution", we employ Bayesian model selection, offering a robust and quantifiable comparison between different analytical models. We believe that this work offers pivotal insights for the analysis of neutron reflectometry and hope that it will contribute to more accurate and information-rich analyses in the future.

==> Table_contrasts.tex <==
\begin{table}
\centering
\arrayrulecolor{black}
\begin{tabular}{>{\hspace{0pt}}m{0.315\linewidth}>{\centering\hspace{0pt}}m{0.094\linewidth}|>{\centering\hspace{0pt}}m{0.067\linewidth}>{\centering\hspace{0pt}}m{0.131\linewidth}|>{\centering\hspace{0pt}}m{0.056\linewidth}>{\centering\hspace{0pt}}m{0.085\linewidth}|>{\centering\hspace{0pt}}m{0.056\linewidth}>{\centering\hspace{0pt}}m{0.056\linewidth}>{\centering\arraybackslash\hspace{0pt}}m{0.069\linewidth}|} 
\arrayrulecolor{black}\cline{3-9}
                                                                                & \multicolumn{1}{>{\hspace{0pt}}m{0.094\linewidth}|}{}             & \multicolumn{2}{>{\centering\hspace{0pt}}m{0.198\linewidth}!{\color{black}\vrule}}{Sample} & \multicolumn{2}{>{\centering\hspace{0pt}}m{0.141\linewidth}|}{Permalloy spin} & \multicolumn{3}{>{\centering\arraybackslash\hspace{0pt}}m{0.181\linewidth}|}{Water}                                                             \\ 
\arrayrulecolor{black}\cline{1-2}\arrayrulecolor{black}\cline{3-9}
\multicolumn{1}{|>{\hspace{0pt}}m{0.315\linewidth}!{\color{black}\vrule}}{Name} & \multicolumn{1}{>{\hspace{0pt}}m{0.094\linewidth}|}{\# contrasts} & \multicolumn{1}{>{\centering\hspace{0pt}}m{0.067\linewidth}|}{Subst.} & Subst. + bilayer   & \multicolumn{1}{>{\centering\hspace{0pt}}m{0.056\linewidth}|}{Up} & Down      & \multicolumn{1}{>{\centering\hspace{0pt}}m{0.056\linewidth}|}{H2O} & \multicolumn{1}{>{\centering\hspace{0pt}}m{0.056\linewidth}|}{D2O} & AuMW  \\ 
\hhline{>{\arrayrulecolor{black}}-->{\arrayrulecolor{black}}------->{\arrayrulecolor{black}}|}
\rowcolor[rgb]{0.859,0.859,0.859} 10contrasts\_H2O\_D2O\_AuMW                   & 10                                                                & ✔️                                                                    & ✔️                 & ✔️                                                                & ✔️        & ✔️                                                                 & ✔️                                                                 & ✔️    \\
8contrasts\_H2O\_D2O                                                            & 8                                                                 & ✔️                                                                    & ✔️                 & ✔️                                                                & ✔️        & ✔️                                                                 & ✔️                                                                 & ~     \\
\rowcolor[rgb]{0.859,0.859,0.859} 4contrasts\_spin\_up\_H2O\_D2O                & 4                                                                 & ✔️                                                                    & ✔️                 & ✔️                                                                & ~         & ✔️                                                                 & ✔️                                                                 & ~     \\
4contrasts\_spin\_down\_H2O\_D2O                                                & 4                                                                 & ✔️                                                                    & ✔️                 & ~                                                                 & ✔️        & ✔️                                                                 & ✔️                                                                 & ~     \\
\rowcolor[rgb]{0.859,0.859,0.859} 4contrasts\_bilayer\_H2O\_D2O                 & 4                                                                 & ~                                                                     & ✔️                 & ✔️                                                                & ✔️        & ✔️                                                                 & ✔️                                                                 & ~     \\
2contrasts\_spin\_up\_H2O                                                       & 2                                                                 & ✔️                                                                    & ✔️                 & ✔️                                                                & ~         & ✔️                                                                 &                                                                    & ~     \\
\rowcolor[rgb]{0.859,0.859,0.859} 2contrasts\_spin\_up\_D2O                     & 2                                                                 & ✔️                                                                    & ✔️                 & ✔️                                                                & ~         & ~                                                                  & ✔️                                                                 & ~     \\
2contrasts\_spin\_up\_bilayer\_H2O\_D2O                                         & 2                                                                 & ~                                                                     & ✔️                 & ✔️                                                                & ~         & ✔️                                                                 & ✔️                                                                 & ~     \\
\rowcolor[rgb]{0.859,0.859,0.859} 2contrasts\_spin\_down\_H2O                   & 2                                                                 & ✔️                                                                    & ✔️                 & ~                                                                 & ✔️        & ✔️                                                                 & ~                                                                  & ~     \\
2contrasts\_spin\_down\_D2O                                                     & 2                                                                 & ✔️                                                                    & ✔️                 & ~                                                                 & ✔️        & ~                                                                  & ✔️                                                                 & ~     \\
\rowcolor[rgb]{0.859,0.859,0.859} 2contrasts\_spin\_down\_bilayer\_H2O\_D2O     & 2                                                                 & ~                                                                     & ✔️                 & ~                                                                 & ✔️        & ✔️                                                                 & ✔️                                                                 & ~     \\
1contrast\_bilayer\_spin\_up\_H2O                                               & 1                                                                 & ~                                                                     & ✔️                 & ✔️                                                                & ~         & ✔️                                                                 &                                                                    & ~     \\
\rowcolor[rgb]{0.859,0.859,0.859} 1contrast\_bilayer\_spin\_up\_D2O             & 1                                                                 & ~                                                                     & ✔️                 & ✔️                                                                & ~         & ~                                                                  & ✔️                                                                 & ~     \\
1contrast\_bilayer\_spin\_down\_H2O                                             & 1                                                                 & ~                                                                     & ✔️                 & ~                                                                 & ✔️        & ✔️                                                                 &                                                                    & ~     \\
\rowcolor[rgb]{0.859,0.859,0.859} 1contrast\_bilayer\_spin\_down\_D2O           & 1                                                                 & ~                                                                     & ✔️                 & ~                                                                 & ✔️        & ~                                                                  & ✔️                                                                 & ~     \\
\hhline{>{\arrayrulecolor[rgb]{0.859,0.859,0.859}}-->{\arrayrulecolor{black}}-->{\arrayrulecolor{black}}->{\arrayrulecolor{black}}->{\arrayrulecolor{black}}-->{\arrayrulecolor{black}}->{\arrayrulecolor{black}}|}
\end{tabular}
\arrayrulecolor{black}
\end{table}
